FAM: Relative Flatness Aware Minimization

Flatness of the loss curve around a model at hand has been shown to empirically correlate with its generalization ability. Optimizing for flatness has been proposed as early as 1994 by Hochreiter and Schmidthuber, and was followed by more recent successful sharpness-aware optimization techniques. Their widespread adoption in practice, though, is dubious because of the lack of theoretically grounded connection between flatness and generalization, in particular in light of the reparameterization curse - certain reparameterizations of a neural network change most flatness measures but do not change generalization. Recent theoretical work suggests that a particular relative flatness measure can be connected to generalization and solves the reparameterization curse. In this paper, we derive a regularizer based on this relative flatness that is easy to compute, fast, efficient, and works with arbitrary loss functions. It requires computing the Hessian only of a single layer of the network, which makes it applicable to large neural networks, and with it avoids an expensive mapping of the loss surface in the vicinity of the model. In an extensive empirical evaluation we show that this relative flatness aware minimization (FAM) improves generalization in a multitude of applications and models, both in finetuning and standard training. We make the code available at github.

==> preamble.tex <==
\RequirePackage{amsthm, amsmath, amssymb}
%\usepackage{algpseudocode,algorithm,algorithmicx}
\usepackage{fancyvrb}

\def\UrlFont{\rm}  
%\usepackage{natbib} 
\usepackage{caption} 
\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage{microtype}
\usepackage{diagbox}
%\usepackage{subfigure}
\usepackage{arydshln} %gives dashed lines in tables
% Packages
\usepackage{latexsym}
%\usepackage[ruled, vlined, nofillcomment, linesnumbered]{algorithm2e}
\usepackage{eda} % The EDA package, includes many default packages
\usepackage{multirow}
%used for stricking out text
\usepackage[normalem]{ulem}



==> sec_notes.tex <==
\section{Notes:}
- check that our measure is properly backpropagatable

- compare regularizing only one layer to multiple layers with our measure (as well as different layers)

- compare with SAM

- include FashionMNIST and SVHN

Argument:

- SAM is great practical success, but theoretical justification doubtful

- instead relative flatness is theoretically sound and outperforms SAM in practice





\section{Experiment Plan}
\subsection{Initial Experiments}
\emph{Michael, Linara}\\
Check on CIFAR10, whether FAM improves generlization.\\
\textbf{Status: }it does improve SOTA on CIFAR10 by from ACC $95.14$ to $95.41$. Now check how it fares without data augmentation.

\subsection{Main Experiments}
\emph{Michael, Linara, Amr}\\
Compare FAM (with neuronwise measure and normal Hessian-trace-based measure).\\
Baselines: SAM (sharpness aware minimization) and no regularization. Other baselines?\\
Datasets: CIFAR10, CIFAR100, something with LSTMs? Skull reconstruction (see below).\\
\textbf{Status: }?


\subsection{Hessian Approximation to Speedup Computation}
\emph{Amr}\\
Test various Hessian approximation methods on trained CIFAR10 network in terms of how well they approximate the (i) whole Hessian, (ii) the trace of the Hessian, (iii) our neuronwise relative flatness measure, and (iv) our trace-based relative flatness measure. In a later stage, test how well regularization works with those approximations.\\
\textbf{Status: }?

 



\textbf{Status: } ?

\subsection{Sampling-based Improvement of FAM}
\emph{Michael, Linara, Amr}\\
In each computation of the regularizer, calculate the correct regularizer, then $k$ times add noise to the weights of the representation and recalculate it. Use the average of all $k+1$ values (or minimum, or maximum, geometric median, average weighted by distance to original weights, etc.).\\
\textbf{Status: }?

\subsection{FedFAM}
\emph{Michael, Amr}\\
Train on CIFAR10 in federated setup. First, calculate regularizer correctly:
in each update step, send model to server and average, send average back to clients; Clients compute Hessian of average model and send it to server; server averages Hessians, computes regularizer, sends it back to clients; clients perform update step.
Look at \citet{qu2022generalized}, might be related.

This is very inefficient. Trivial improvement: only use local FAM regularization. 

Better improvement: communicate in every update step but use local regularizer values as samples like in the sampling-based improvement of FAM. This is theoretically wrong, bc. local datasets are different and local networks are entirely different (in particular the parts before the representation). Still, this could work in practice.\\
\textbf{Status: }?
